The Local Group L-Band Survey: The First Measurements of Localized Cold Neutral Medium Properties in the Low-Metallicity Dwarf Galaxy NGC 6822

Measuring the properties of the cold neutral medium (CNM) in low-metallicity galaxies provides insight into heating and cooling mechanisms in early Universe-like environments. We report detections of two localized atomic neutral hydrogen (HI) absorption features in NGC 6822, a low-metallicity (0.2 Z$_{\odot}$) dwarf galaxy in the Local Group. These are the first unambiguous CNM detections in a low-metallicity dwarf galaxy outside the Magellanic Clouds. The Local Group L-Band Survey (LGLBS) enabled these detections due to its high spatial (15 pc for HI emission) and spectral (0.4 \kms) resolution. We introduce LGLBS and describe a custom pipeline to search for HI absorption at high angular resolution and extract associated HI emission. A detailed Gaussian decomposition and radiative transfer analysis of the NGC 6822 detections reveals five CNM components, with key properties: a mean spin temperature of 32$\pm$6 K, a mean CNM column density of 3.1$\times$10$^{20}$ cm$^{-2}$, and CNM mass fractions of 0.33 and 0.12 for the two sightlines. Stacking non-detections does not reveal low-level signals below our median optical depth sensitivity of 0.05. One detection intercepts a star-forming region, with the HI absorption profile encompassing the CO (2$-$1) emission, indicating coincident molecular gas and a depression in high-resolution HI emission. We also analyze a nearby sightline with deep, narrow HI self-absorption dips, where the background warm neutral medium is attenuated by intervening CNM. The association of CNM, CO, and H$\alpha$ emissions suggests a close link between the colder, denser HI phase and star formation in NGC 6822.

==> authors.tex <==
%% please add your name, affiliation, and ORCID here

\author[0000-0001-9504-7386]{Nickolas~M.~Pingel}
\affiliation{University of Wisconsin–Madison, Department of Astronomy, 475 N Charter St, Madison, WI 53703, USA}

\author[0009-0005-1781-5665]{Hongxing Chen}
\affiliation{University of Wisconsin–Madison, Department of Astronomy, 475 N Charter St, Madison, WI 53703, USA}

\author[0000-0002-3418-7817]{Sne\v{z}ana Stanimirovi\'c}
\affiliation{University of Wisconsin–Madison, Department of Astronomy, 475 N Charter St, Madison, WI 53703, USA}

\author[0000-0001-9605-780X]{Eric W. Koch}
\affiliation{Center for Astrophysics $\mid$ Harvard & Smithsonian, 60 Garden St., 02138 Cambridge, MA, USA}

\author[0000-0002-4781-7291]{Sumit K. Sarbadhicary}
\affiliation{Department of Physics, The Ohio State University, Columbus, Ohio 43210, USA}
\affiliation{Center for Cosmology \& Astro-Particle Physics, The Ohio State University, Columbus, Ohio 43210, USA}
\affiliation{Department of Astronomy, The Ohio State University, Columbus, Ohio 43210, USA}

\author[0000-0003-1356-1096]{Elizabeth Tarantino}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive, Baltimore, MD 21218, USA}

\author[0000-0002-3106-7676]{Jennifer Donovan Meyer}
\affiliation{National Radio Astronomy Observatory, 520 Edgemont Rd., Charlottesville, VA 22968, USA}

\author[0000-0002-1264-2006]{Julianne J.~Dalcanton}
\affiliation{Center for Computational Astrophysics, Flatiron Institute, 162 Fifth Avenue, New York, NY 10010, USA}
\affiliation{Department of Astronomy, Box 351580, University of Washington, Seattle, WA 98195, USA}

email: Laura, Julianna

\author{LGLBS Friends}


